A Higher-Order Swiss Army Infinitesimal Jackknife

Cross validation (CV) and the bootstrap are ubiquitous model-agnostic tools for assessing the error or variability of machine learning and statistical estimators. However, these methods require repeatedly re-fitting the model with different weighted versions of the original dataset, which can be prohibitively time-consuming. For sufficiently regular optimization problems the optimum depends smoothly on the data weights, and so the process of repeatedly re-fitting can be approximated with a Taylor series that can be often evaluated relatively quickly. The first-order approximation is known as the "infinitesimal jackknife" in the statistics literature and has been the subject of recent interest in machine learning for approximate CV. In this work, we consider high-order approximations, which we call the "higher-order infinitesimal jackknife" (HOIJ). Under mild regularity conditions, we provide a simple recursive procedure to compute approximations of all orders with finite-sample accuracy bounds. Additionally, we show that the HOIJ can be efficiently computed even in high dimensions using forward-mode automatic differentiation. We show that a linear approximation with bootstrap weights approximation is equivalent to those provided by asymptotic normal approximations. Consequently, the HOIJ opens up the possibility of enjoying higher-order accuracy properties of the bootstrap using local approximations. Consistency of the HOIJ for leave-one-out CV under different asymptotic regimes follows as corollaries from our finite-sample bounds under additional regularity assumptions. The generality of the computation and bounds motivate the name "higher-order Swiss Army infinitesimal jackknife."

==> acknowledgements.tex <==
\paragraph{Acknowledgements.} We thank anonymous reviewers for their helpful
comments and suggestions. We are grateful to Nelle Varoquaux for her help with
the genomics experiments. This research was supported in part by DARPA
(FA8650-18-2-7832), an ARO YIP award, an NSF CAREER award, and the CSAIL-MSR
Trustworthy AI Initiative. Ryan Giordano was supported by the Gordon and Betty
Moore Foundation through Grant GBMF3834 and by the Alfred P. Sloan Foundation
through Grant 2013-10-27 to the University of California, Berkeley. Runjing Liu
was supported by the NSF Graduate Research Fellowship.


==> choosing_omega.tex <==
Recall that \defref{wdom} requires $\allthetadom$ to contain $\thetaw[w]$, but
that we do not know $\thetaw[w]$ in advance. In theory, one could define
$\allthetadom$ to contain all plausible values of $\theta$, but at the cost of
extremely loose constants. In this section we discuss a practical resolution to
this chicken-and-egg problem.  Although we do not observe $\thetaw[w]$, the HOIJ
$\thetaij$ provides an estimate of $\thetaw[w]$ with calculable error $\errij$
for a tentative guess of $\allthetadom$.  Consequently, we might imagine finding
the smallest $\allthetadom$ such that we know that $\thetaij$ plus its error---
and hence $\thetaw[w]$---is contained within $\allthetadom$.  In this section,
we formalize this intuitive approach.

For simplicity, let us define $\allthetadomb := \{\theta: \norm{\theta -
\thetaone}_2 \le B \}$ for a positive scalar $B$. When using $\allthetadomb$, the
quantities $\cop$, $\mk$, and $\deltak$, all being suprema over $\allthetadomb$,
are monotonically increasing in  $B$ without loss of generality.  In turn, both
$\errij$ and $\cset$ in \condref{theta_small} will depend on $B$ in a
monotonically increasing way, which we emphasize by writing $\errij(w, B)$ and
$\cset(B)$.

Because our error bounds are exact, if $B$ is large enough to contain both
$\thetaij$ and its error $\errij(w, B)$, but small enough that we can satisfy
\condref{theta_small}, then we know that $\allthetadomb$ also contains $\thetaw$ as
well.  We formalize this in the following lemma.

%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%
\begin{lem}\lemlabel{thetadom_ball}%\seeproof{thetadom_ball}
%
Fix some $B > 0$, $0 < \deltabound < 1$, and let $\allthetadom = \allthetadomb$.
Let \assuref{diffable}, \assuref{bounded}, \assuref{convexity}, and
\assuref{complexity} hold with corresponding $\cset(B)$ and $\errij[\kij](\wt,
B)$. Let $\errij[\kij](\wt, B)$ be the error as given by \thmref{thetaij_error}.
(Note that we have not assumed \assuref{thetadom} or \condref{theta_small},
so $\errij[\kij](\wt, B)$ may not control $\norm{\thetaij - \thetaw[w]}_2$.
% TODO: should we use different notation for this?)

If $B$ satisfies
%
\begin{align*}
\cset(B) &\le \deltabound \quad\textrm{and} \\
B &> \sup_{\wt \in \wdom} \left( \norm{\thetaij[\kij][\wt] -
    \thetaone}_2 + \errij[\kij](\wt, B)\right),
\end{align*}
%
then $\allthetadomb$ satisfies \assuref{thetadom}, \condref{theta_small} holds,
and $\norm{\thetaij - \thetaw[w]}_2 \le \errij[\kij](\wt, B)$.
%
\begin{proof}\prooflabel{thetadom_ball}
    We first observe that $\allthetadom[\wt] \subseteq \allthetadom$, if
    \allassums hold for $w$ then they hold for all $\wt \in \wdom$, and

\end{proof}
%
\end{lem}
%
%%%%%%%%%%%%%%%%%%%%%%%

Note that $B = 0$ cannot satisfy \lemref{thetadom_ball} (as long as
$\thetaij[\kij] \ne \thetaone$).  Furthermore, if $B = 0$ does not satisfy
$\cset(B) \le 1$, then there will be no $B$ that satisfies
\lemref{thetadom_ball} because $\cset(B)$ is increasing in $B$. Consequently, by
starting at $B = 0$ and increasing $B$ until \lemref{thetadom_ball} is first
satisfied is guaranteed to find the smallest $L_2$ ball that satisfies
$\defref{wdom}$.

% \begin{algorithm}
% \caption{Finding $\allthetadom$}%\label{euclid}
% \begin{algorithmic}
% \Procedure{EvaluateB}{$\thetaone$, $\thetaij$, $\errij(\cdot)$, $\cset(\cdot)$ }
%     \State \Return
%         $\cset(B) \le \deltabound$ and
%         $\norm{\thetaij[\kij] - \thetaone}_2 + \errij[\kij](B)$
% \EndProcedure
%
% \State done = False
% \State B = 0
% \While{Not done}
%     \If \Call{EvaluateB}{B}
%         \State \Return $\allthetadomb$
%     \Else
%         \State B $\gets$ \Call{Increase}{B}
%     \EndIf
% \EndWhile
% \end{algorithmic}
% \end{algorithm}

